Seeing My Future: Predicting Situated Interaction Behavior in Virtual Reality

Virtual and augmented reality systems increasingly demand intelligent adaptation to user behaviors for enhanced interaction experiences. Achieving this requires accurately understanding human intentions and predicting future situated behaviors - such as gaze direction and object interactions - which is vital for creating responsive VR/AR environments and applications like personalized assistants. However, accurate behavioral prediction demands modeling the underlying cognitive processes that drive human-environment interactions. In this work, we introduce a hierarchical, intention-aware framework that models human intentions and predicts detailed situated behaviors by leveraging cognitive mechanisms. Given historical human dynamics and the observation of scene contexts, our framework first identifies potential interaction targets and forecasts fine-grained future behaviors. We propose a dynamic Graph Convolutional Network (GCN) to effectively capture human-environment relationships. Extensive experiments on challenging real-world benchmarks and live VR environment demonstrate the effectiveness of our approach, achieving superior performance across all metrics and enabling practical applications for proactive VR systems that anticipate user behaviors and adapt virtual environments accordingly.

==> sec/notation.tex <==
\newcommand{\misscite}{\textcolor{red}{[C]~}}
\newcommand{\missref}{\textcolor{red}{[R]~}}

\makeatletter
\newcommand{\thickhline}{
    \noalign {\ifnum 0=`}\fi \hrule height 1pt
    \futurelet \reserved@a \@xhline
}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} 
\def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\aka{a.k.a\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


\acrodef{sota}[SOTA]{State-of-the-Art}
\acrodef{hoi}[HOI]{Human Object Interaction}
\acrodef{eisp}[EISP]{Electromagnetic Inverse Scattering Problems}
\acrodef{mlp}[MLP]{multilayer perceptron}
\acrodef{gcn}[GCN]{graph convolutional network}
\acrodef{dgcn}[D-GCN]{dynamic graph convolutional network}
\acrodef{dct}[DCT]{discrete cosine transform}
\acrodef{idct}[IDCT]{Inverse Discrete Cosine Transform}
\acrodef{gt}[GT]{groud-truth}


\newcommand{\loss}{\mathcal{L}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\B}{B} 
\newcommand{\D}{D}
\newcommand{\Nobj}{N} 
\newcommand{\Nnode}{n}
\newcommand{\Demb}{d} 
 
\newcommand{\history}[1]{\mathbf{#1}} 
\newcommand{\gazeHist}{\mathbf{g}} 
\newcommand{\headRotHist}{\mathbf{R}_\text{head}} 
\newcommand{\headPosHist}{\mathbf{P}_\text{head}}
\newcommand{\handPosHist}{\mathbf{P}_\text{hand}} 
\newcommand{\objCenterHist}{\mathbf{P}_\text{center}}
\newcommand{\objBoxHist}{\mathbf{P}_\text{bbox}}
\newcommand{\frameHist}{T_\text{h}}
 
\newcommand{\objClipFeat}{\mathbf{F}_{\text{clip}}} 
\newcommand{\dimClip}{\D_{\text{clip}}}
 
\newcommand{\pred}[1]{\hat{#1}} 
\newcommand{\gazePred}{\pred{\gazeHist}} 
\newcommand{\headRotPred}{\pred{\mathbf{R}}_{\text{head}}} 
\newcommand{\headPosPred}{\pred{\mathbf{P}}_{\text{head}}} 
\newcommand{\handPosPred}{\pred{\mathbf{P}}_{\text{hand}}} 
\newcommand{\objCenterPred}{\pred{\mathbf{P}}_\text{center}} 
\newcommand{\interactLabel}{\mathbf{p}} 
\newcommand{\interactLabelPred}{\pred{\interactLabel}} 
\newcommand{\interactLabelRawPred}{\pred{\interactLabel}_\text{int}}
\newcommand{\headVelPred}{\pred{\mathbf{V}}_{\text{head}}}
\newcommand{\handVelPred}{\pred{\mathbf{V}}_{\text{hand}}}
\newcommand{\objCenterVelPred}{\pred{\mathbf{V}}_{\text{center}}}
\newcommand{\framePred}{T_\text{f}}

\newcommand{\topk}{K}
\newcommand{\fgaze}{\mathbf{F}_{\text{gaze}}}
\newcommand{\fheadrot}{\mathbf{F}_{\text{head\_rot}}}
\newcommand{\fheadpos}{\mathbf{F}_{\text{head\_pos}}}
\newcommand{\fhandpos}{\mathbf{F}_{\text{hand\_pos}}}
\newcommand{\fpose}{\mathbf{F}_{\text{human}}}
\newcommand{\fglobal}{\mathbf{F}_{\text{global}}}
\newcommand{\fobj}{\mathbf{F}_{\text{obj}}}
\newcommand{\fobjupdate}{\mathbf{H}_{\text{obj}}}
\newcommand{\fglobalupdate}{\mathbf{H}_{\text{global}}}
\newcommand{\fgazeupdate}{\mathbf{H}_{\text{gaze}}}
\newcommand{\ftopk}{\mathbf{F}_{\text{k}}}

\newcommand{\fdct}{f_{\text{dct}}}
\newcommand{\fmlpselect}{f_{\text{p}}}
\newcommand{\fmlpgaze}{f_{\text{g}}}
\newcommand{\fgcn}{f_{\text{gcn}}}
\newcommand{\layer}{\text{L}}
\newcommand{\layere}{\layer_{\text{e}}}
\newcommand{\layerd}{\layer_{\text{d}}}
\newcommand{\layeri}{\layer_{\text{i}}}


\newcommand{\AdjD}{\mathbf{A}_\text{D}} 
\newcommand{\AdjT}{\mathbf{A}_\text{T}} 
\newcommand{\AdjS}{\mathbf{A}_\text{S}}
\newcommand{\AdjNorm}{\mathbf{D}}
\newcommand{\WeightMat}{\mathbf{W}}
\newcommand{\NodeFeat}{\mathbf{X}} 
\newcommand{\anglegaze}{\mathbf{\theta}_\text{g}}
\newcommand{\distgaze}{\mathbf{d}_{\text{g}}}
\newcommand{\distpose}{\mathbf{d}_{\text{p}}}
\newcommand{\distobj}{\mathbf{d}_{\text{o}}}
\newcommand{\Adjg}{\mathbf{A}_{\text{g}}}
\newcommand{\Adjo}{\mathbf{A}_{\text{o}}}
\newcommand{\Adjp}{\mathbf{A}_{\text{p}}}
\newcommand{\hiddenFeat}{\mathbf{H}}

\newcommand{\lossgaze}{\loss_{\text{gaze}}}
\newcommand{\losspos}{\loss_{\text{pos}}}
\newcommand{\lossrot}{\loss_{\text{rot}}}
\newcommand{\lossprob}{\loss_{\text{prob}}}
\newcommand{\lossvel}{\loss_{\text{vel}}}
\newcommand{\lossobjpos}{\loss_{\text{center}}}
\newcommand{\lossselect}{\loss_{\text{int}}}
\newcommand{\losslabel}{\loss_{\text{state}}}
 
\newcommand{\groundtruth}[1]{\Tilde{\mathbf{#1}}} 
\newcommand{\gazeGT}{\groundtruth{\gazeHist}} 
\newcommand{\headRotGT}{\groundtruth{R}_{\text{head}}}
\newcommand{\headPosGT}{\groundtruth{P}_{\text{head}}}
\newcommand{\handPosGT}{\groundtruth{P}_{\text{hand}}}
\newcommand{\objCenterGT}{\groundtruth{P}_{\text{center}}}
\newcommand{\interactLabelGT}{\groundtruth{\interactLabel}}
\newcommand{\headVelGT}{\groundtruth{V}_{\text{head}}}
\newcommand{\handVelGT}{\groundtruth{V}_{\text{hand}}}
\newcommand{\objCenterVelGT}{\groundtruth{V}_{\text{center}}}

